Split, Send, Reassemble: A Formal Specification of a CAN Bus Protocol Stack

We present a formal model for a fragmentation and a reassembly protocol running on top of the standardised CAN bus, which is widely used in automotive and aerospace applications. Although the CAN bus comes with an in-built mechanism for prioritisation, we argue that this is not sufficient and provide another protocol to overcome this shortcoming.

==> eptcsdata.tex <==
\providecommand{\firstpage}{14}
\providecommand{\publicationstatus}{H. Hermanns, P. H\"ofner (Eds.): Models for \\
Formal Analysis of Real Systems (MARS 2017)\\
EPTCS 244, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.244.2}{10.4204/EPTCS.244.2}}
\pdfoutput=1

